Federated Semi-Supervised Learning with Inter-Client Consistency & Disjoint Learning

While existing federated learning approaches mostly require that clients have fully-labeled data to train on, in realistic settings, data obtained at the client-side often comes without any accompanying labels. Such deficiency of labels may result from either high labeling cost, or difficulty of annotation due to the requirement of expert knowledge. Thus the private data at each client may be either partly labeled, or completely unlabeled with labeled data being available only at the server, which leads us to a new practical federated learning problem, namely Federated Semi-Supervised Learning (FSSL). In this work, we study two essential scenarios of FSSL based on the location of the labeled data. The first scenario considers a conventional case where clients have both labeled and unlabeled data (labels-at-client), and the second scenario considers a more challenging case, where the labeled data is only available at the server (labels-at-server). We then propose a novel method to tackle the problems, which we refer to as Federated Matching (FedMatch). FedMatch improves upon naive combinations of federated learning and semi-supervised learning approaches with a new inter-client consistency loss and decomposition of the parameters for disjoint learning on labeled and unlabeled data. Through extensive experimental validation of our method in the two different scenarios, we show that our method outperforms both local semi-supervised learning and baselines which naively combine federated learning with semi-supervised learning. The code is available at https://github.com/wyjeong/FedMatch.

==> figures/figure_params.tex <==
\begin{figure*}
\small
    \centering
    \begin{tabular}{c c}
        \hspace{-0.1in}
        \includegraphics[width=.51\textwidth]{figures/images/fig-lc.pdf}
        &\includegraphics[width=.46\textwidth]{figures/images/fig-ls.pdf} 
        \\
        \hspace{-0.25in}
        (a) Labels-at-Client Scenario & 
        (b) Labels-at-Server Scenario \\
    \end{tabular}
    \vspace{-0.10in}
    \caption{\small\textbf{Illustration of Parameter Decomposition for Disjoint Learning}  (a) Labels-at-Client scenario: Active local model $l_a$ learns both $\sigma^{l_a}$ and $\psi^{l_a}$. Then, server aggregates $\sigma^{l_{1:A}}$ and $\psi^{l_{1:A}}$, respectively, while selecting the top-$H$ $\psi^{h_{1:H}}$ based on model similarity. (b) Labels-at-Server scenario: The global model $G$ learns $\sigma^G$ at server and the active local clients $l_{1:A}$ learn $\psi^{l_{1:A}}$. Once clients update their $\psi^{l_{1:A}}$ to the server, server selects the top-$H$ most similar $\psi^{h_{1:H}}$.}
    \label{fig:params}
    \vspace{-0.15in}
\end{figure*}

% \caption{\small\textbf{Illustration of Parameter Decomposition for Disjoint Learning}  (a) \textbf{Labels-at-Client scenario}: Active local model $l_a$ at the current round learns both $\sigma^{l_a}$ and $\psi^{l_a}$ on labeled and unlabeled data. Once the clients update their weights to the server, server aggregates $\sigma^{l_{1:A}}$ and $\psi^{l_{1:A}}$, respectively, while selecting the top-$H$ $\psi^{h_{1:H}}$ based on model similarity. Then, the server broadcasts the aggregated $\sigma$ and $\psi$, as well as the $H$ selected $\psi^{h_{1:H}}$ to next available clients ($H$=$2$). (b) \textbf{Labels-at-Server scenario}: The global model $G$ learns $\sigma^G$ on labeled data at server and the active local clients $l_{1:A}$ at the current round learn $\psi^{l_{1:A}}$ on unlabeled data. Once clients update their $\psi^{l_{1:A}}$ to the server, server selects the top-$H$ most similar $\psi^{h_{1:H}}$. Then, server broadcasts its learned $\sigma_G$ as well as the aggregated $\psi$ and top-$H$ similar $\psi^{h_{1:H}}$ to the next available clients ($H$=$2$).}

==> figures/figure_streaming.tex <==
% \begin{figure}
%     \begin{minipage}{.4\textwidth}
%         \includegraphics[width=.85\textwidth]{figures/images/fig-bs-all.eps}
%     \end{minipage}
%     \vspace{-0.1in} 
%     \noindent
%     \begin{minipage}{.6\textwidth}
%         \hspace{-0.35in}
%         \small{
%             \begin{tabular}{cccccc}
%             \hline
%                 \hline
%                 \multicolumn{5}{l}{\textbf{Fashion-MNIST, Streaming-NonIID Tasks ($K$=$10$,$F$=$1$,$H$=$2$,$T$=$10$)}} 
%                 \\ \hline 
                
%                 \multicolumn{1}{c||}{}
%                 & \multicolumn{2}{c||}{\emph{Labels-at-Client}}
%                 & \multicolumn{2}{c}{\emph{Labels-at-Server}}
%                 \\ \hline
                
%                 \multicolumn{1}{c||}{\textbf{Methods}}
%                 & \multicolumn{1}{c|}{\textbf{Acc.(\%)}}
%                 & \multicolumn{1}{c||}{\textbf{Cost(C)}}
%                 & \multicolumn{1}{c|}{\textbf{Acc.(\%)}}
%                 & \multicolumn{1}{c}{\textbf{Cost(C)}}
%                 \\ \hline
                
%                 \multicolumn{1}{l||}{Local SL} 
%                 & \multicolumn{1}{c|}{47.23 \tiny{$\pm$ 0.01}} 
%                 & \multicolumn{1}{c||}{100 \% } 
%                 & \multicolumn{1}{c|}{47.87 \tiny{$\pm$ 0.01}} 
%                 & \multicolumn{1}{c}{100 \% } 
%                 \\ 
                
%                 \multicolumn{1}{l||}{Local UDA}
%                 & \multicolumn{1}{c|}{47.54 \tiny{$\pm$ 0.01}} 
%                 & \multicolumn{1}{c||}{100 \% } 
%                 & \multicolumn{1}{c|}{48.01 \tiny{$\pm$ 0.01}}
%                 & \multicolumn{1}{c}{100 \% } 
%                 \\ 
                
%                 \multicolumn{1}{l||}{Local FixMatch} 
%                 & \multicolumn{1}{c|}{35.27 \tiny{$\pm$ 0.01}} 
%                 & \multicolumn{1}{c||}{100 \% } 
%                 & \multicolumn{1}{c|}{35.20 \tiny{$\pm$ 0.01}}
%                 & \multicolumn{1}{c}{100 \% } 
%                 \\ 
%                 \hdashline   
                
%                 \multicolumn{1}{l||}{FedPrx-SL} 
%                 & \multicolumn{1}{c|}{34.93 \tiny{$\pm$ 0.01}} 
%                 & \multicolumn{1}{c||}{100 \% } 
%                 & \multicolumn{1}{c|}{36.67 \tiny{$\pm$ 0.01}}
%                 & \multicolumn{1}{c}{100 \% } 
%                 \\   
                
%                 \multicolumn{1}{l||}{FedProx-UDA} 
%                 & \multicolumn{1}{c|}{32.33 \tiny{$\pm$ 0.02}} 
%                 & \multicolumn{1}{c||}{100 \% } 
%                 & \multicolumn{1}{c|}{36.27 \tiny{$\pm$ 0.01}}
%                 & \multicolumn{1}{c}{100 \% } 
%                 \\ 
%                 \multicolumn{1}{l||}{FedProx-FixMatch} 
%                 & \multicolumn{1}{c|}{36.83 \tiny{$\pm$ 0.02}} 
%                 & \multicolumn{1}{c||}{100 \% } 
%                 & \multicolumn{1}{c|}{36.37 \tiny{$\pm$ 0.04}}
%                 & \multicolumn{1}{c}{100 \% } 
%                 \\ \hdashline
                
%                 \multicolumn{1}{l||}{\textbf{FedMatch-S}} 
%                 & \multicolumn{1}{c|}{\textbf{38.43} \tiny{$\pm$ 0.01}} 
%                 & \multicolumn{1}{c||}{\textbf{102 \%} } 
%                 & \multicolumn{1}{c|}{\textbf{38.83} \tiny{$\pm$ 0.01}}
%                 & \multicolumn{1}{c}{\textbf{102 \%} } 
%                 % & \multicolumn{1}{c|}{xx.xx  }
%                 % & \multicolumn{1}{c}{100 \% } 
%                 \\ 
                
%                 \multicolumn{1}{l||}{\textbf{FedMatch-D} } 
%                 & \multicolumn{1}{c|}{\textbf{41.67} \tiny{$\pm$ 0.01}} 
%                 & \multicolumn{1}{c||}{\textbf{177 \%} } 
%                 & \multicolumn{1}{c|}{\textbf{41.97} \tiny{$\pm$ 0.01}} 
%                 & \multicolumn{1}{c}{\textbf{177 \%} } 
%                 % & \multicolumn{1}{c|}{xx.xx  } 
%                 % & \multicolumn{1}{c}{xx \% } 
%                 \\ \hline
%             \end{tabular}
            
%         }
%     \end{minipage}
%     \caption{\small{\textbf{Performance Comparison on Streaming-NonIID Tasks} }}
%     \label{fig:streaming}
% \end{figure}


==> sections/3_approach.tex <==

\vspace{-0.1in}
\section{Federated Matching}
\vspace{-0.1in}
We now describe our \emph{Federated Matching (FedMatch)} algorithm to tackle the federated semi-supervised learning problems. The overall learning procedure of FedMatch is illustrated in Figure~\ref{fig:iccs} and~\ref{fig:params}, and we describe its core components in detail in the following subsections.

\input{figures/figure_iccs}

\vspace{-0.1in}
\paragraph{Inter-Client Consistency Loss}
\label{inter-client-consistency}
Consistency regularization~\citep{xie2019unsupervised,sohn2020fixmatch,berthelot2019mixmatch,berthelot2019remixmatch} is one of most popular approaches to learn from unlabeled examples in a semi-supervised learning setting. Conventional consistency-regularization methods enforce the predictions from the augmented examples and original (or weakly augmented) instances to output the same class label,  $||p_{\bsy\theta}(\textbf{y}|\pi(\textbf{u}))-p_{\bsy\theta}(\textbf{y}|\pi(\textbf{u}))||^2_2$, where $\pi(\cdot)$ is a stochastic transformation function. Based on the assumption that class semantics are unaffected by small input perturbations, these methods basically ensures consistency of the prediction across the multiple perturbations of \emph{same input}. For our federated semi-supervised learning method, we additionally propose a novel consistency loss that regularizes the \emph{models} learned at multiple clients to output the same prediction. This novel consistency loss for FSSL, \emph{inter-client consistency} loss, is defined as follows:
% \vspace{-0.05in}
\begin{equation}
\begin{split}
\frac{1}{H}\sum_{j=1}^H \textrm{KL}[p^*_{\bsy\theta^{\textrm{h}_j}}(\textbf{y}|\textbf{u)}||p_{\bsy\theta^{l}}(\textbf{y}|\textbf{u})]
\end{split}
\end{equation}
% \vspace{-0.05in}
\noindent where $p^*_{\bsy\theta^{h}}(\textbf{y}|\textbf{x})$ are helper agents that are selected from the server based on model similarity to the client (which we describe later), that are not trained at the client (* denotes that we freeze the parameters). The server selects and broadcasts $H$ helper agents at each communication round. We also use data-level consistency regularization at each local client similarly to FixMatch~\citep{sohn2020fixmatch}. Our final consistency regularization term $\Phi(\cdot)$ can be written as follows:
\vspace{-0.1in}
\begin{equation}
\begin{split}
\Phi(\cdot)=\textrm{CrossEntropy}(\hat{\textbf{y}}, p_{\bsy\theta^{l}}(\textbf{y}|\pi(\textbf{u}))) +\frac{1}{H} \sum_{j=1}^H \textrm{KL}[p^*_{\bsy\theta^{\textrm{h}_j}}(\textbf{y}|\textbf{u})||p_{\bsy\theta^{l}}(\textbf{y}|\textbf{u})]
\end{split}
\end{equation}%p^*_{\theta^{l}}(\textbf{y}
\noindent where $\pi(\textbf{u})$ performs RandAugment~\citep{DBLP:journals/corr/abs-1909-13719} on unlabeld instance $\textbf{u}$. $\hat{\textbf{y}}$ is our novel pseudo-labeling technique, which we refer to as the \textit{agreement-based} pseudo label, defined as follows:
\vspace{-0.1in}
\begin{equation}
\begin{split}
\hat{\textbf{y}} = \textrm{Max}(\mathbbm{1}(p^*_{\bsy\theta^{l}}(\textbf{y}|\textbf{u}))+\sum_{j=1}^{H}\mathbbm{1}(p^*_{\bsy\theta^{h_j}}(\textbf{y}|\textbf{u})))
\end{split}
\end{equation}
\noindent where $\mathbbm{1}(\cdot)$ produces one-hot labels with given softmax values , and $\textrm{Max}(\cdot)$ outputs one-hot labels on the class that has the maximum agreements. We discard instances with low-confident predictions below confidence threshold $\tau$ when generating pseudo-labels. We then perform standard cross-entropy minimization with the pseudo-label $\hat{\textbf{y}}$. We select the $H$ helper agents $p^*_{\bsy\theta^{\textrm{h}_{j:H}}}(\textbf{y}|\textbf{u})$ for each client as the most relevant models from other clients. Specifically, we represent each model by its prediction $\textbf{m}$ on the same arbitrary input $\textbf{a}$ located at server (we use random Gaussian noise), such that $\textbf{m}^{l}$= $p_{\bsy\theta^{l}}(\textbf{m}|\textbf{a})$. The server tries to keep and update all model embeddings $\textbf{m}^{1:K}$ from clients once each client updates its weights to server, and creates \emph{K-Dimensional Tree (KD Tree)} on $\textbf{m}$ in the current round $r$ for nearest neighbor search to rapidly select the $H$ helper agents for each client in the next round $r+1$. If a certain client has not yet updated its weights to server in the previous step, then server simply omits sending helpers to the client. 

\input{figures/figure_params}
\vspace{-0.1in}
\paragraph{Parameter Decomposition for Disjoint Learning} In the standard semi-supervised learning approaches, learning on labeled and unlabeled data is simultaneously done with a shared set of parameters. However, since this is inapplicable to the disjoint learning scenario (Figure~\ref{fig:concepts} (b)) and may result in forgetting of knowledge of labeled data, we separate the supervised and unsupervised learning via the decomposition of model parameters into two sets of parameters, one for supervised learning and another for unsupervised learning. To this end, we decompose our model parameters $\theta$ into two variables, $\sigma$ for supervised learning and $\psi$ for unsupervised learning, such that $\theta=\sigma+\psi$. We perform standard supervised learning on $\sigma$, while keeping $\psi$ fixed during training, by minimizing the loss term as follows: 
\begin{equation}
\begin{split}
\textrm{minimize}~\mathcal{L}_s(\sigma) = \lambda_s \textrm{CrossEntropy}(\textbf{y}, p_{\sigma+\psi^*}(\textbf{y}|\textbf{x}))
\end{split}
\end{equation}
\noindent where $\textbf{x}$ and $\textbf{y}$ are from labeled set $\mathcal{S}$. For the standard scenario, $\mathcal{L}_s(\sigma)$ is computed at client, while calculated at server for the disjoint scenario, depending on the availability of $\mathcal{S}$.
For learning on unlabeled data, we perform unsupervised learning conversely on $\psi$, while keeping $\sigma$ fixed for the learning phase, by minimizing the consistency loss terms as follows:
\begin{equation}
\begin{split}
\textrm{minimize}~\mathcal{L}_u(\psi) = \lambda_{\textrm{ICCS}}\Phi_{\sigma^*+\psi}(\cdot) + \lambda_{L_2}||\sigma^*-\psi||_2^2 +\lambda_{L_1}||\psi||_1
\end{split}
\end{equation}
\noindent where all $\lambda$s are hyper-parameters to control the learning ratio between the terms. We additionally add $L_2$- and $L_1$-Regularization on $\psi$ such that $\psi$ is sparse, while not drifting far from knowledge that $\sigma$ has learned. To sum up, our decomposition technique allows us: 
\vspace{-0.1in}
\begin{itemize}[leftmargin=0.20in]
    \item \textbf{Preservation Reliable Knowledge from Labeled Data}: We empirically find that learning on both labeled and unlabeled data with a single set of parameters may result in the model to forget about what it learned from the labeled data (see Figure~\ref{fig:analysis} (c)). Our method can effectively prevent the \emph{inter-task interference} via utilizing disjoint parameters only for supervised learning.
    \item \textbf{Reduction of Communication Costs}: Sparsity on the unsupervised parameter $\psi$ allows to reduce communication cost. In addition, we further minimize the cost by subtracting the learned knowledge for each parameter, such that $\Delta\psi=\psi_{r}^{l}-\psi_{r}^{G}$ and  $\Delta\sigma=\sigma_{r}^{l}-\sigma_{r}^{G}$, and transmit only the differences $\Delta\psi$ and $\Delta\sigma$ as sparse matrices for both client-to-server and server-to-client costs.
    \item \textbf{Disjoint Learning}: In federated semi-supervised learning, labeled data can be located at either client or server, which requires the model's learning procedure to be flexible. Our decomposition technique allows the model for the supervised training to be done separately elsewhere. 
\end{itemize}

% This sparse parameters enable efficient communications between clients and server. 
% especially when $\sigma$ is located at server, as only sparse $\psi$ needs to be sent.



==> sections/7_acknowledgements.tex <==
\section{Acknowledgements}


==> sections/fssl.tex <==




